ControlTraj: Controllable Trajectory Generation with Topology-Constrained Diffusion Model

Generating trajectory data is among promising solutions to addressing privacy concerns, collection costs, and proprietary restrictions usually associated with human mobility analyses. However, existing trajectory generation methods are still in their infancy due to the inherent diversity and unpredictability of human activities, grappling with issues such as fidelity, flexibility, and generalizability. To overcome these obstacles, we propose ControlTraj, a Controllable Trajectory generation framework with the topology-constrained diffusion model. Distinct from prior approaches, ControlTraj utilizes a diffusion model to generate high-fidelity trajectories while integrating the structural constraints of road network topology to guide the geographical outcomes. Specifically, we develop a novel road segment autoencoder to extract fine-grained road segment embedding. The encoded features, along with trip attributes, are subsequently merged into the proposed geographic denoising UNet architecture, named GeoUNet, to synthesize geographic trajectories from white noise. Through experimentation across three real-world data settings, ControlTraj demonstrates its ability to produce human-directed, high-fidelity trajectory generation with adaptability to unexplored geographical contexts.

==> Figures/figures.tex <==
% 自定义颜色
\definecolor{cmp1}{RGB}{0,129,218}
\definecolor{amp1}{RGB}{29,254,179}
\definecolor{ump1}{RGB}{62,254,94}
\definecolor{gmp1}{RGB}{194,254,0}
\definecolor{imp1}{RGB}{254,129,0}
\definecolor{xmp1}{RGB}{212,0,0}

% mark 样式 *, x , +, |, o, asterisk, star, 10-pointed star, oplus, oplus*, otimes, otimes*, square, square*, triangle, triangle*, diamond, halfdiamond*, halfsquare*, right*, left*, Mercedes star, Mercedes star flipped, halfcircle, halfcircle*, pentagon, pentagon*,



\begin{figure}
\begin{tikzpicture}
\begin{axis}[
width=8cm, 
height=6cm,
axis line style={black, thick}, % 设置轴线的颜色和粗细
inner axis line style={dotted}, % 设置内轴线的样式
outer axis line style={solid}, % 设置外轴线的样式
legend pos=north east,
ymajorgrids=true,
grid style=dashed,
title={xxxxxxx},
xlabel={XLabel},
ylabel={Ylabel},
xmin=0, xmax=100,
ymin=0, ymax=120,
xtick={0,20,40,60,80,100},
ytick={0,20,40,60,80,100,120},
]
\addplot[
    color=orange, % 更改颜色为橙色
    dashed, % 更改线条样式
    mark=star, % 更改标记
    line width=1.5pt, % 增加线条粗细
    mark size=2.5pt % 增加标记大小
    ]
    coordinates {
    (0,  80)
    (10, 80)
    (20, 80)
    (30, 80)
    (40, 80)
    (60, 80)
    (80, 80)
    (100, 80)
    };
\addplot[
    color=xmp1,
    solid,
    mark=diamond,
    line width= 1.5pt,
    ]   
    coordinates {
    (0,  40)
    (10, 40)
    (20, 40)
    (30, 40)
    (40, 40)
    (60, 40)
    (80, 40)
    (100, 40)
    };
    \legend{Legend-A, Legend-B}
\end{axis}
\end{tikzpicture}
\caption{Line graph of density over time}
\end{figure}




\begin{figure}
\begin{tikzpicture}
\begin{axis}[
width=8cm, 
height=6cm,
axis line style={black, thick}, % 设置轴线的颜色和粗细
inner axis line style={dotted}, % 设置内轴线的样式
outer axis line style={solid}, % 设置外轴线的样式
% x tick label style={
%     /pgf/number format/1000 sep=},
ylabel={Year},
enlargelimits=0.15, % 增大柱子与坐标轴的间隙
% legend pos=north east,
legend style={at={(0.7, 0.95)}, % 调整图例位置
    anchor=north,legend columns=-1},
ybar=1pt, % 调整柱子之间的间距
bar width=15pt, % 调整柱子的宽度
% ymin=380000, % 可以调整以确保所有的柱子都能完整显示
% nodes near coords, % 在柱子顶部显示数值
]
\addplot[
    fill=cmp1!50, % 柱子的填充颜色，50%
    draw=black, % 柱子的边框颜色
] 
coordinates {
(2012, 4084) 
(2011, 4048)
(2010, 4170) 
(2009, 4156)
};
\addplot[
    fill=xmp1!50, % 柱子的填充颜色，50%
    draw=black, % 柱子的边框颜色
]
coordinates {
(2012, 3850) 
(2011, 3907)
(2010, 3943) 
(2009, 3972)
};
\legend{Men,Women}
\end{axis}
\end{tikzpicture}
\end{figure}




\begin{table*}[t]
    % \scriptsize
    % \fontsize{7.3pt}{8.4pt}\selectfont
    \caption{Performance comparison of different generative approaches. }
    \centering
    \begin{tabular}{lcccccc} 
    \toprule
      \multirow{2}{*}[\multirowoffset]{Methods} & \multicolumn{3}{c}{Chengdu} & \multicolumn{3}{c}{Xi'an}  \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
     & Density ($\downarrow$) & Trip ($\downarrow$) & Length ($\downarrow$) & Density ($\downarrow$) & Trip ($\downarrow$) & Length ($\downarrow$) \\ 
    \cmidrule(lr){1-7}
   RP  & 0.0698 & 0.0835 & 0.2337 & 0.0543  & 0.0744 & 0.2067  \\
    GP  & 0.1365 & 0.1590 & 0.1423  & 0.0928 & 0.1013  & 0.2164  \\
    \cmidrule(lr){1-7}
VAE  & 0.0148 & 0.0452   & 0.0383 & 0.0237 & 0.0608 & 0.0497   \\
TrajGAN  & 0.0125 & 0.0497 & 0.0388  & 0.0220 & 0.0512  & 0.0386  \\
DP-TrajGAN & 0.0117	& 0.0443 & 0.0221  & 0.0207 & 0.0498 & 0.0436  \\
Diffwave  & 0.0145 & 0.0253 & 0.0315 &  0.0213 & 0.0343 & 0.0321 \\
% Diff-LSTM  & 0.0068 & 0.0199 & 0.0217 & 0.0142  & 0.0195 & 0.0259  \\
DiffTraj  & 0.0055 & 0.0154 & 0.0169  & 0.0126  & 0.0165 & 0.0203 \\
RI-DiffTraj-25\%  & 0.0068 & 0.0199 & 0.0217 & 0.0142  & 0.0195 & 0.0259  \\
    \bottomrule
    \end{tabular}
    \label{tab:comp}
\end{table*}
